MambaAD: Exploring State Space Models for Multi-class Unsupervised Anomaly Detection

Recent advancements in anomaly detection have seen the efficacy of CNN- and transformer-based approaches. However, CNNs struggle with long-range dependencies, while transformers are burdened by quadratic computational complexity. Mamba-based models, with their superior long-range modeling and linear efficiency, have garnered substantial attention. This study pioneers the application of Mamba to multi-class unsupervised anomaly detection, presenting MambaAD, which consists of a pre-trained encoder and a Mamba decoder featuring (Locality-Enhanced State Space) LSS modules at multi-scales. The proposed LSS module, integrating parallel cascaded (Hybrid State Space) HSS blocks and multi-kernel convolutions operations, effectively captures both long-range and local information. The HSS block, utilizing (Hybrid Scanning) HS encoders, encodes feature maps into five scanning methods and eight directions, thereby strengthening global connections through the (State Space Model) SSM. The use of Hilbert scanning and eight directions significantly improves feature sequence modeling. Comprehensive experiments on six diverse anomaly detection datasets and seven metrics demonstrate state-of-the-art performance, substantiating the method's effectiveness. The code and models are available at https://lewandofskee.github.io/projects/MambaAD.

==> sec/ref.tex <==
{\small
\bibliographystyle{abbrvnat}
\bibliography{ref}
}


==> sec/test.tex <==
\section{More Quantitative Results for Each Category on The MVTec-AD Dataset for Single-class Anomaly Detection.}

\begin{table*}[htbp]
  \centering
  \caption{Comparison with SoTA methods on\textbf{ MVTec-AD} dataset for \textbf{single-class} anomaly detection with AU-ROC/AP/F1\_max metrics.}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{p{3em}<{\centering} p{3.25em}<{\centering}p{6.2em}<{\centering} p{6.2em}<{\centering} p{6.2em}<{\centering} p{6.2em}<{\centering} p{6.2em}<{\centering} p{6.2em}<{\centering} p{6.2em}<{\centering} p{7em}<{\centering}}
    \toprule
    \multicolumn{2}{c}{Method~$\rightarrow$} & RD4AD~\cite{deng2022anomaly} & UniAD~\cite{you2022unified} & SimpleNet~\cite{liu2023simplenet}  & DeSTSeg~\cite{zhang2023destseg}  & PatchCore~\cite{roth2022towards} & \cellcolor{tab_ours}{MambaAD} \\
    \cline{1-2}
    \multicolumn{2}{c}{Category~$\downarrow$} & CVPR'22 & NeurlPS'22 & CVPR'23 & CVPR'23 & CVPR'22& \cellcolor{tab_ours}{ours}\\
    \hline
    \multicolumn{1}{c}{\multirow{10}[1]{*}{\begin{turn}{-90}Objects\end{turn}}} & \multicolumn{1}{c}{Bottle} & \textbf{100.}/\textbf{100.}/\textbf{100.}&\textbf{100.}/\textbf{100.}/\textbf{100.}&99.9/\textbf{100.}/99.2&\textbf{100.}/\textbf{100.}/\textbf{100.}&\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_ours}\textbf{100.}/\textbf{100.}/\textbf{100.} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Cable} & \cellcolor{tab_others}94.8/97.0/89.7&\cellcolor{tab_others}97.9/98.7/93.8&\cellcolor{tab_others}99.6/99.7/97.3&\cellcolor{tab_others}97.1/98.4/93.3&\cellcolor{tab_others}\textbf{99.8}/\textbf{99.9}/\textbf{98.9}&\cellcolor{tab_ours}98.5/99.1/95.1 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Capsule}  & \textbf{98.4}/\textbf{99.7}/97.3&87.1/95.3/95.2&97.2/99.2/\textbf{98.6}&97.4/99.5/96.8&97.4/99.4/98.2&\cellcolor{tab_ours}97.8/99.5/97.2 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Hazelnut} & \cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_others}99.7/99.8/98.6&\cellcolor{tab_others}99.0/99.4/97.2&\cellcolor{tab_others}99.7/99.8/99.3&\cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_ours}\textbf{100.}/\textbf{100.}/\textbf{100.} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Metal Nut}  & 99.9/\textbf{100.}/99.5&98.7/99.7/98.4&99.9/\textbf{100.}/99.5&99.7/99.9/98.9&99.9/\textbf{100.}/99.5&\cellcolor{tab_ours}\textbf{100.}/\textbf{100.}/99.5 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Pill}  & \cellcolor{tab_others}97.5/99.6/97.1&\cellcolor{tab_others}96.0/99.3/95.8&\cellcolor{tab_others}\textbf{98.6}/\textbf{99.7}/\textbf{97.9}&\cellcolor{tab_others}96.2/99.3/95.7&\cellcolor{tab_others}96.6/99.4/96.5&\cellcolor{tab_ours}95.3/99.1/95.3 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Screw} & 97.7/99.2/95.9&87.7/93.0/93.1&97.5/99.2/95.1&92.3/97.5/90.9&\textbf{98.1}/\textbf{99.3}/\textbf{97.}5&\cellcolor{tab_ours}97.6/99.1/97.1 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Toothbrush} & \cellcolor{tab_others}93.3/97.2/95.2&\cellcolor{tab_others}88.1/94.8/93.8&\cellcolor{tab_others}99.4/99.8/98.4&\cellcolor{tab_others}99.7/99.9/98.4&\cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_ours}96.1/98.4/95.2 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Transistor} & 98.4/97.7/93.8&\textbf{100.}/\textbf{100.}/\textbf{100.}&99.9/99.9/98.7&98.5/98.2/94.7&\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_ours}\textbf{100.}/\textbf{100.}/\textbf{100.} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Zipper}  & \cellcolor{tab_others}98.3/99.5/97.9&\cellcolor{tab_others}90.6/96.5/93.9&\cellcolor{tab_others}99.8/99.9/99.6&\cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_others}99.6/99.9/98.7&\cellcolor{tab_ours}98.6/99.6/97.5 \\
    \hline
    \multicolumn{1}{c}{\multirow{5}[1]{*}{\begin{turn}{-90}Textures\end{turn}}} & \multicolumn{1}{c}{Carpet}  & 99.7/99.9/98.3&99.4/99.8/98.9&99.1/99.7/98.3&99.3/99.8/97.7&98.5/99.6/97.1&\cellcolor{tab_ours}\textbf{100.}/\textbf{100.}/\textbf{100.} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Grid} & \cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_others}97.6/99.3/96.6&\cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_others}99.7/99.9/99.1&\cellcolor{tab_ours}\textbf{100.}/\textbf{100.}/\textbf{100.} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Leather} & \textbf{100.}/\textbf{100.}/\textbf{100.}&\textbf{100.}/\textbf{100.}/\textbf{100.}&\textbf{100.}/\textbf{100.}/\textbf{100.}&\textbf{100.}/\textbf{100.}/\textbf{100.}&\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_ours}\textbf{100.}/\textbf{100.}/\textbf{100.}\\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Tile}  & \cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{100.}&\cellcolor{tab_others}95.8/98.2/95.8&\cellcolor{tab_others}99.9/99.9/98.8&\cellcolor{tab_others}\textbf{100.}/\textbf{100.}/99.4&\cellcolor{tab_others}99.0/99.7/98.8&\cellcolor{tab_ours}97.5/99.1/94.7 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Wood}  & 99.5/99.8/98.3&97.9/99.4/95.9&99.9/\textbf{100.}/99.2&99.3/99.8/98.4&99.1/99.7/97.5&\cellcolor{tab_ours}99.6/99.9/99.2 \\
    \hline
    \multicolumn{2}{c}{\cellcolor{tab_others}Mean} & \cellcolor{tab_others}98.5/99.3/97.5&\cellcolor{tab_others}95.8/98.9/96.7&\cellcolor{tab_others}\textbf{99.3}/\textbf{99.8}/98.5&\cellcolor{tab_others}98.6/99.5/97.6&\cellcolor{tab_others}99.2/\textbf{99.8}/\textbf{98.8}&\cellcolor{tab_ours}98.7/99.6/98.1 \\
    \bottomrule
    \end{tabular}%
  }
  \label{tab:sgmvtecsp}%
\end{table*}%

\begin{table*}[htbp]
  \centering
  \caption{Comparison with SoTA methods on \textbf{MVTec-AD} dataset for \textbf{single-class }anomaly localization with AU-ROC/AP/F1\_max/AU-PRO metrics.}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{cccccccc}
    \toprule
    \multicolumn{2}{c}{Method~$\rightarrow$} & RD4AD~\cite{deng2022anomaly} & UniAD~\cite{you2022unified} & SimpleNet~\cite{liu2023simplenet}  & DeSTSeg~\cite{zhang2023destseg}  & PatchCore~\cite{roth2022towards} & \cellcolor{tab_ours}MambaAD \\
    \cline{1-2}
    \multicolumn{2}{c}{Category~$\downarrow$} & CVPR'22 & NeurlPS'22 & CVPR'23 & CVPR'23 & CVPR'22& \cellcolor{tab_ours}(ours) \\
    \hline
    \multicolumn{1}{c}{\multirow{10}[1]{*}{\begin{turn}{-90}Objects\end{turn}}} & \multicolumn{1}{c}{Bottle} &  98.6/75.9/74.1/95.8&98.3/73.6/70.7/94.4&98.0/70.4/72.7/88.8&\textbf{99.3}/\textbf{91.0}/\textbf{84.3}/94.0&98.5/77.7/75.2/94.9&\cellcolor{tab_ours}98.8/79.7/76.6/\textbf{96.1} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Cable} & \cellcolor{tab_others}96.8/51.3/57.3/88.8&\cellcolor{tab_others}97.4/54.8/56.9/87.7&\cellcolor{tab_others}97.4/\textbf{66.8}/60.0/87.7&\cellcolor{tab_others}95.8/55.0/52.8/82.4&\cellcolor{tab_others}\textbf{98.4}/66.3/\textbf{65.1}/92.5&\cellcolor{tab_ours}98.0/54.4/61.7/\textbf{93.4}\\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Capsule} & 98.9/48.1/49.9/95.3&98.0/35.2/40.1/86&98.9/42.5/49.1/92.8&98.8/\textbf{52.4}/\textbf{57.9}/71.6&\textbf{99.0}/44.7/50.9/91.7&\cellcolor{tab_ours}98.6/45.0/47.5/\textbf{94.3} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Hazelnut} & \cellcolor{tab_others}98.8/59.6/60.8/\textbf{96.5}&\cellcolor{tab_others}98.3/55.0/56.1/92.8&\cellcolor{tab_others}97.9/46.2/50.3/78.9&\cellcolor{tab_others}\textbf{99.4}/\textbf{84.5}/\textbf{79.0}/90.6&\cellcolor{tab_others}98.7/53.5/59.2/89.7&\cellcolor{tab_ours}99.0/61.8/63.9/95.8  \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Metal Nut} & 96.9/75.3/79.5/\textbf{94.1}&94.4/55.8/68.8/77.8&98.8/91.6/86.6/84.0&\textbf{99.2}/\textbf{95.0}/\textbf{88.7}/95.0&98.3/86.9/85.1/91.4&\cellcolor{tab_ours}97.1/78.3/80.6/93.6 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Pill} & \cellcolor{tab_others}97.6/66.6/66.7/\textbf{95.9}&\cellcolor{tab_others}95.2/45.9/51.9/92.2&\cellcolor{tab_others}98.5/79.5/72.6/92.5&\cellcolor{tab_others}\textbf{98.9}/\textbf{87.9}/\textbf{79.6}/56.6&\cellcolor{tab_others}97.8/77.8/72.9/94.1&\cellcolor{tab_ours}97.3/64.5/66.0/95.8 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Screw} & \textbf{99.5}/44.6/47.2/96.9&98.4/15.5/23.6/91.3&99.3/35.0/38.8/95.2&97.3/\textbf{54.2}/\textbf{53.3}/53.6&\textbf{99.5}/36.5/40.1/96.6&\cellcolor{tab_ours}\textbf{99.5}/52.2/51.7/\textbf{97.6} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Toothbrush} & \cellcolor{tab_others}99.0/51.8/60.9/92.0&\cellcolor{tab_others}98.5/42.6/52.1/84.6&\cellcolor{tab_others}98.5/41.7/52.9/\textbf{92.4}&\cellcolor{tab_others}\textbf{99.5}/\textbf{78.2}/\textbf{73.7}/90.8&\cellcolor{tab_others}98.6/38.3/52.3/92.3&\cellcolor{tab_ours}99.0/51.1/60.7/92.3 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Transistor} & 90.6/52.8/54.9/80.8&\textbf{98.8}/\textbf{79.5}/\textbf{75.8}/\textbf{94.5}&96.8/67.4/62.1/91.1&88.1/63.6/60.0/80.9&96.2/66.4/61.5/89.8&\cellcolor{tab_ours}96.8/69.7/67.5/91.6 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Zipper}  & \cellcolor{tab_others}98.7/53.0/59.0/94.6&\cellcolor{tab_others}96.5/35.5/43.4/89.3&\cellcolor{tab_others}98.9/64.3/65.4/\textbf{95.5}&\cellcolor{tab_others}\textbf{99.2}/\textbf{85.7}/\textbf{77.4}/84.3&\cellcolor{tab_others}98.9/62.9/66.1/94.3&\cellcolor{tab_ours}98.1/55.6/58.8/94.8 \\
    \hline
    \multicolumn{1}{c}{\multirow{5}[1]{*}{\begin{turn}{-90}Textures\end{turn}}} & \multicolumn{1}{c}{Carpet} & 99.1/60.1/60.9/95.6&98.5/52.1/53.3/94.9&98.0/43.2/47.8/87.9&98.2/\textbf{77.5}/\textbf{72.5}/94.9&99.1/64.1/63.0/94.8&\cellcolor{tab_ours}\textbf{99.2}/63.0/63.4/\textbf{97.0} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Grid}  & \cellcolor{tab_others}99.3/45.2/47.7/96.3&\cellcolor{tab_others}94.3/24.3/31.5/85.8&\cellcolor{tab_others}98.8/34.7/39.3/93.9&\cellcolor{tab_others}\textbf{99.5}/\textbf{62.5}/\textbf{63.5}/93.8&\cellcolor{tab_others}98.8/31.0/35.3/94.2&\cellcolor{tab_ours}99.2/48.9/48.8/\textbf{97.3}\\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Leather} & 99.3/44.7/46.7/97.9&99.1/38.5/41.9/98.1&99.2/41.7/45.6/95.7&\textbf{99.8}/\textbf{74.9}/\textbf{69.6}/96.9&99.3/46.3/46.7/96.8&\cellcolor{tab_ours}99.3/47.5/49.5/\textbf{98.6} \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\cellcolor{tab_others}Tile}  & \cellcolor{tab_others}95.1/48.6/59.7/85.1&\cellcolor{tab_others}90.2/40.4/48.7/77.1&\cellcolor{tab_others}97.2/69.8/68.8/89.7&\cellcolor{tab_others}\textbf{99.4}/\textbf{94.6}/\textbf{87.1}/89.1&\cellcolor{tab_others}95.8/55.0/64.7/\textbf{90.0}&\cellcolor{tab_ours}93.1/42.8/52.3/80.3 \\
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{Wood} & 94.8/48.6/49.5/91.6&93.5/38.6/43.9/85.2&94.0/45.6/48.1/82.5&\textbf{98.4}/\textbf{84.5}/\textbf{77.5}/90.9&95.0/50.2/50.9/85.3&\cellcolor{tab_ours}93.9/44.2/47.7/\textbf{92.1} \\
    \hline
    \multicolumn{2}{c}{\cellcolor{tab_others}Mean} & \cellcolor{tab_others}97.5/55.1/58.3/93.1&\cellcolor{tab_others}96.6/45.8/50.6/88.8&\cellcolor{tab_others}98.0/56.0/57.3/89.9&\cellcolor{tab_others}\textbf{98.1}/\textbf{76.1}/\textbf{71.8}/84.4&\cellcolor{tab_others}\textbf{98.1}/57.2/59.3/92.6&\cellcolor{tab_ours}97.8/57.2/59.8/\textbf{94.0} \\
    \bottomrule
    \end{tabular}
  }
  \label{tab:sgmvtecpx}%
\end{table*}%


\begin{table*}[htbp]
  \centering
   \caption{Comparison with SoTA methods on \textbf{VisA} dataset for \textbf{single-class} anomaly detection with AU-ROC/AP/F1\_max metrics.}
  \resizebox{1.\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
    Method~$\rightarrow$ & RD4AD~\cite{deng2022anomaly} & UniAD~\cite{you2022unified} & SimpleNet~\cite{liu2023simplenet}  & DeSTSeg~\cite{zhang2023destseg}  & PatchCore~\cite{roth2022towards} & \cellcolor{tab_ours}MambaAD \\
    \cline{1-1}
    Category~$\downarrow$ & CVPR'22 & NeurlPS'22 & CVPR'23 & CVPR'23 & CVPR'22& \cellcolor{tab_ours}(ours) \\
    \hline
    pcb1  & 95.9/95.6/92.8&91.9/90.9/87.2&\textbf{98.9}/\textbf{98.9}/\textbf{96.0}&94.9/92.5/92.0&97.7/97.1/94.9&\cellcolor{tab_ours}96.0/95.1/93.8 \\
    \cellcolor{tab_others}pcb2  & \cellcolor{tab_others}96.5/96.2/92.1&\cellcolor{tab_others}92.2/92.3/84.8&\cellcolor{tab_others}\textbf{98.8}/\textbf{98.8}/\textbf{93.9}&\cellcolor{tab_others}96.6/94.7/93.4&\cellcolor{tab_others}97.7/98.2/93.3&\cellcolor{tab_ours}97.1/96.8/91.9 \\
    pcb3  & 96.2/96.1/91.1&90.9/91.3/86.2&\textbf{98.9}/\textbf{98.8}/\textbf{95.1}&97.0/97.3/91.7&98.5/98.5/93.5&\cellcolor{tab_ours}97.8/98.0/92.7 \\
    \cellcolor{tab_others}pcb4  & \cellcolor{tab_others}\textbf{100.}/\textbf{100.}/\textbf{99.5}&\cellcolor{tab_others}98.8/98.6/96.1&\cellcolor{tab_others}99.3/99.0/97.6&\cellcolor{tab_others}99.3/99.3/94.8&\cellcolor{tab_others}99.8/99.8/97.5&\cellcolor{tab_ours}99.7/99.7/97.5 \\
    \hline
    macaroni1 & 92.1/90.2/85.4&87.5/83.3/79.6&\textbf{94.8}/\textbf{92.7}/\textbf{89.0}&82.8/75.1/77.2&91.3/85.9/87.0&\cellcolor{tab_ours}91.2/88.4/84.1 \\
    \cellcolor{tab_others}macaroni2 & \cellcolor{tab_others}\textbf{86.1}/80.3/\textbf{80.2}&\cellcolor{tab_others}83.1/\textbf{82.5}/76.4&\cellcolor{tab_others}83.4/77.0/70.4&\cellcolor{tab_others}72.8/66.1/69.2&\cellcolor{tab_others}75.2/60.6/59.4&\cellcolor{tab_ours}81.8/78.9/77.7 \\
    capsules & 89.7/94.2/87.7&79.1/88.7/79.0&90.1/93.3/86.4&85.3/91.5/83.6&77.7/83.2/74.4&\cellcolor{tab_ours}\textbf{91.4}/\textbf{94.6}/\textbf{90.5} \\
    \cellcolor{tab_others}candle & \cellcolor{tab_others}94.6/94.7/89.4&\cellcolor{tab_others}96.5/96.5/89.3&\cellcolor{tab_others}92.3/85.6/86.9&\cellcolor{tab_others}94.6/95.1/87.2&\cellcolor{tab_others}92.2/85.3/84.4&\cellcolor{tab_ours}\textbf{97.7}/\textbf{97.7}/\textbf{92.1} \\
    \hline
    cashew & \textbf{96.9}/\textbf{98.6}/93.4&91.9/96.1/90.3&94.1/96.2/90.9&73.8/87.2/81.3&91.2/93.5/89.2&\cellcolor{tab_ours}95.7/97.6/\textbf{93.7}\\
    \cellcolor{tab_others}chewinggum &\cellcolor{tab_others}98.8/99.4/96.3&\cellcolor{tab_others}97.4/98.8/94.8&\cellcolor{tab_others}98.6/99.3/\textbf{96.9}&\cellcolor{tab_others}97.1/98.8/95.9&\cellcolor{tab_others}97.9/98.8/95.4&\cellcolor{tab_ours}\textbf{99.0}/\textbf{99.5}/96.1 \\
    fryum &94.8/97.7/91.7&85.5/92.6/86.0&96.4/98.0/\textbf{93.5}&91.7/96.0/88.6&95.0/96.7/89.8&\cellcolor{tab_ours}\textbf{96.5}/\textbf{98.3}/92.5 \\
    \cellcolor{tab_others}pipe\_fryum &\cellcolor{tab_others}99.7/99.8/98.5&\cellcolor{tab_others}91.9/95.4/90.8&\cellcolor{tab_others}\textbf{99.8}/\textbf{99.9}/\textbf{99.0}&\cellcolor{tab_others}99.3/99.6/97.5&\cellcolor{tab_others}99.1/99.5/97.5&\cellcolor{tab_ours}99.2/99.6/97.6 \\
    \hline
    Mean  & 95.1/95.2/91.5&90.6/92.3/86.7&\textbf{95.4}/94.8/91.3&90.4/91.1/87.7&92.8/91.4/88.0&\cellcolor{tab_ours}95.3/\textbf{95.3}/\textbf{91.7}\\
    \bottomrule
    \end{tabular}
  }
  \label{tab:sgvisasp}%
\end{table*}%

\begin{table*}[htbp]
  \centering
  \caption{Comparison with SoTA methods on \textbf{VisA} dataset for \textbf{single-class} anomaly localization with AU-ROC/AP/F1\_max/AU-PRO metrics.}
  \resizebox{1\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule
    Method~$\rightarrow$ & RD4AD~\cite{deng2022anomaly} & UniAD~\cite{you2022unified} & SimpleNet~\cite{liu2023simplenet}  & DeSTSeg~\cite{zhang2023destseg}  & PatchCore~\cite{roth2022towards} & \cellcolor{tab_ours}MambaAD \\
    \cline{1-1}
    Category~$\downarrow$ & CVPR'22 & NeurlPS'22 & CVPR'23 & CVPR'23 & CVPR'22& \cellcolor{tab_ours}(ours) \\
    \midrule
    pcb1  & 99.7/71.2/68.4/94.8&99.2/53.0/56.2/86.7&99.6/87.7/78.4/89.6&99.4/61.5/62.8/76.9&\textbf{99.8}/\textbf{91.8}/\textbf{85.9}/94.7&\cellcolor{tab_ours}\textbf{99.8}/72.5/67.4/\textbf{94.9} \\
    \cellcolor{tab_others}pcb2  & \cellcolor{tab_others}98.8/16.2/24.0/90.1&\cellcolor{tab_others}97.1/ \;5.8/13.0/80.8&\cellcolor{tab_others}98.2/11.9/22.2/87.7&\cellcolor{tab_others}98.9/\textbf{20.0}/\textbf{30.1}/\textbf{91.5}&\cellcolor{tab_others}98.7/12.5/22.8/89.9&\cellcolor{tab_ours}\textbf{98.9}/10.1/19.5/90.7 \\
    pcb3  & 99.2/26.4/29.6/92.0&98.2/14.9/23.0/80.3&99.3/45.5/45.4/92.5&98.7/31.3/33.1/40.4&\textbf{99.4}/\textbf{48.1}/\textbf{47.3}/89.2&\cellcolor{tab_ours}99.3/25.7/27.9/\textbf{92.8} \\
    \cellcolor{tab_others}pcb4  &\cellcolor{tab_others}98.4/39.7/40.9/89.1&\cellcolor{tab_others}97.5/20.8/29.4/82.0&\cellcolor{tab_others}97.5/40.6/45.5/80.6&\cellcolor{tab_others}96.7/27.5/37.5/66.2&\cellcolor{tab_others}98.2/42.1/45.8/82.2&\cellcolor{tab_ours}\textbf{98.7}/\textbf{47.6}/\textbf{47.0}/\textbf{90.9} \\
    \midrule
    macaroni1 & 99.6/\textbf{21.0}/\textbf{31.1}/95.4&99.0/\;6.8/13.5/95.8&99.6/ \;7.0/11.1/98.5&98.7/17.3/25.3/53.4&\textbf{99.7}/ \;7.8/13.5/98.4&\cellcolor{tab_ours}99.6/18.7/27.8/\textbf{96.8} \\
    \cellcolor{tab_others}macaroni2 & \cellcolor{tab_others}\textbf{99.5}/\textbf{10.9}/\textbf{18.7}/\textbf{95.9}&\cellcolor{tab_others}98.2/ \;3.8/10.3/95.3&\cellcolor{tab_others}98.4/ \;3.9/ \;8.8/94.8&\cellcolor{tab_others}99.0/ \;8.6/18.2/68.8&\cellcolor{tab_others}98.8/ \;4.9/ \;7.6/94.5&\cellcolor{tab_ours}99.3/10.8/16.2/\textbf{95.9} \\
    capsules &\textbf{99.6}/61.1/59.5/92.8&98.4/44.8/49.4/76.6&98.8/52.8/56.2/89.6&98.9/49.6/51.0/90.0&99.4/\textbf{65.2}/\textbf{65.6}/89.8&\cellcolor{tab_ours}99.3/\textbf{65.2}/62.5/\textbf{93.1} \\
    \cellcolor{tab_others}candle & \cellcolor{tab_others}98.9/22.6/33.7/94.5&\cellcolor{tab_others}98.9/16.7/26.2/94.9&\cellcolor{tab_others}98.4/13.1/22.2/90.2&\cellcolor{tab_others}99.0/\textbf{31.1}/\textbf{36.7}/78.7&\cellcolor{tab_others}\textbf{99.3}/18.7/27.2/96.7&\cellcolor{tab_ours}98.7/19.9/30.5/\textbf{95.1}\\
    \midrule
    cashew & 95.4/53.0/56.2/89.8&99.2/64.6/64.3/85.5&98.9/62.3/62.6/78.5&\textbf{99.0}/\textbf{80.1}/\textbf{74.9}/89.2&98.7/58.8/60.0/\textbf{91.8}&\cellcolor{tab_ours}97.5/58.9/59.3/86.9\\
    \cellcolor{tab_others}chewinggum & \cellcolor{tab_others}98.8/54.5/\textbf{59.1}/82.6&\cellcolor{tab_others}98.7/48.0/48.5/81.2&\cellcolor{tab_others}98.4/19.5/35.7/\textbf{86.0}&\cellcolor{tab_others}98.8/24.6/38.8/82.9&\cellcolor{tab_others}\textbf{98.9}/43.0/44.2/81.1&\cellcolor{tab_ours}98.4/\textbf{56.5}/56.2/80.6 \\
    fryum & 96.6/44.2/49.5/90.3&97.1/43.4/51.5/73.8&91.1/37.9/46.0/85.0&95.0/\textbf{51.8}/52.3/70.2&92.6/38.3/45.9/89.1&\cellcolor{tab_ours}\textbf{97.0}/48.1/\textbf{52.9}/\textbf{91.1} \\
    \cellcolor{tab_others}pipe\_fryum &\cellcolor{tab_others}99.0/51.0/55.5/93.7&\cellcolor{tab_others}99.3/56.9/63.7/90.7&\cellcolor{tab_others}98.9/59.6/60.4/91.5&\cellcolor{tab_others}\textbf{99.7}/\textbf{89.2}/\textbf{82.6}/50.7&\cellcolor{tab_others}98.9/58.7/58.8/\textbf{96.4}&\cellcolor{tab_ours}98.9/51.1/54.7/94.0\\
    \midrule
    Mean  & 98.6/39.3/43.8/91.7&98.4/31.6/37.4/85.3&98.1/36.8/41.2/88.7&98.5/\textbf{41.1}/\textbf{45.3}/71.6&98.5/40.8/43.7/91.1&\cellcolor{tab_ours}\textbf{98.8}/40.4/43.5/\textbf{91.9}\\
    \bottomrule
    \end{tabular}
  }
  \label{tab:sgvisapx}%
\end{table*}%

